Mining Clues from Incomplete Utterance: A Query-enhanced Network for Incomplete Utterance Rewriting

Incomplete utterance rewriting has recently raised wide attention. However, previous works do not consider the semantic structural information between incomplete utterance and rewritten utterance or model the semantic structure implicitly and insufficiently. To address this problem, we propose a QUEry-Enhanced Network (QUEEN). Firstly, our proposed query template explicitly brings guided semantic structural knowledge between the incomplete utterance and the rewritten utterance making model perceive where to refer back to or recover omitted tokens. Then, we adopt a fast and effective edit operation scoring network to model the relation between two tokens. Benefiting from proposed query template and the well-designed edit operation scoring network, QUEEN achieves state-of-the-art performance on several public datasets.

==> files/methodology_old.tex <==
\section{Methodology}
\noindent
\textbf{Overview} Our Queen-ATT mainly consists of two modules: query template construction module (Sec.~\ref{sec:query template}) and multi-head attention module (Sec.~\ref{sec:model architecture}). 

The former module aims to generate query sentences for incomplete utterances from two linguistic perspective, i.e., ellipsis-oriented query and coreference-oriented query to cope with ellipsis and coreference problems respectively. 
These queries explicitly enhance the input data with semantic structure information.
The latter module tries to capture the semantic structural relations between words by constructing two edit operation matrices and applying attention mechanism on them.
Our goal is to learn a model to generate correct edit operations on these two matrices so as to convert the incomplete utterance into rewritten complete one. 
% Here, we use two edit operation matrices called substitution matrix and insertion matrix. The substitution matrix is used to tackle the co-reference utterance and the insertion matrix is used for ellipsis utterance. Two edition operation matrix share the same dimention of $2 \times L \times L$,  where $L$ is the token length of input and $Y^{t}_{m,n}$ indicates the edit type $t \in \{substitute, insert\}$ between $m$-th token and $n$-th token.
% % different from \citet{qian2020incomplete}, 
% %\footnote{Method for obtaining the expected supervision are shown in Appendix.}
% In this way, we can find the semantic relationship between each token pair completely. We can also obtain relative position information using relative position coding, instead of using additional LSTM as \citet{qian2020incomplete}.
% During the decoding time, if $Y_{i,m,n}$  equals to $1$, that means edit operation $i$ should to be performed between $c_m$ and $c_n$. For example as shown in Figure \ref{Fig_1}, there are two kind of edit types: \textit{Substitute} means replacing the character with another corresponding character; \textit{Insert} aims to insert the character before a certain character.


\subsection{Query Template Construction Module} % Module
\label{sec:query template}
\noindent
By observing incomplete and rewritten utterance pairs in existing datasets, we find that pronouns in the incomplete utterance often need to be replaced by entities or concepts in dialogue history, such as the ``这样'' (this) in Table~\ref{tab_1}. And ellipsis often occurs in some specific positions of incomplete utterance without pronoun, conforming to certain syntactic structure. In this module, we aims to encode the above two prior linguistic knowledge into the input of our model. The query template is constructed as follows: 

\noindent
\textbf{Pronouns Matching} \quad We use a manual collection to match pronouns in incomplete utterances. Once the match is successful, we use the \texttt{[UNK]} token to replace the pronoun that appears in the incomplete utterance, and we regard this new utterance as the query. For example, we transfer the incomplete utterance ``她是谁'' (Who is she) to the query ``\texttt{[UNK]}是谁'' (Who is \texttt{[UNK]})

\noindent
\textbf{Ellipsis Detection} \quad Once the match fails, dependency parsing will be performed on the incomplete utterance. As most complete utterances have an SVO (Subject-Verb-Object) structure, we use the SVO structure to determine where the ellipsis is possible. When there is not the V-O (Verb-Object) structure after parsing, we insert an \texttt{[UNK]} at the end of the incomplete utterance as the query. 
When the S-V (Subject-Verb) structure doesn't exist after parsing, we insert an \texttt{[UNK]} at the beginning of the incomplete utterance as the query. 
In other cases, we insert \texttt{[UNK]} at both the beginning and end of the incomplete utterance as the query.
As the incomplete utterance ``李明曾经是'' (Li Ming used to be) without pronoun or V-O structure, we transfer it to the query ``李明曾经是\texttt{[UNK]}'' (Li Ming used to be \texttt{[UNK]}).


\subsection{Multi-head Attention Module}
\label{sec:model architecture}
\noindent
The dialogue session $s=(u_1,...,u_N)$ contains $N$ utterances and $u_N$ is the latest utterance that needs to be rewritten. We append the designed query in the beginning of $s$ to get $s' = ({\rm query}, u_1,...,u_N)$. 
We concatenate $s'$ with an \texttt{[END]} token to produce a sequence $C=(c_1,...,c_L)$ with $L$ tokens $c$.

Since pre-trained language models have been proven to be effective on several tasks, we employ Bert \citep{DBLP:conf/naacl/DevlinCLT19} to model the sequence $c = (c_1,c_2,...,c_L)$. Each token $c_j$ is represented using
\begin{align}
h_j = Bert(c_j)
\end{align}
$h_j$ denotes the embedding of token $c_j$.

After encoding, we get the embedding sequence $H=(h_1,h_2,...,h_L)$. Our model attempts to predict whether there is an edit relationship between each token pair. We simplify multi-head attention mechanism \citep{DBLP:conf/nips/VaswaniSPUJGKP17} to model the relationship as fellows,
\begin{align}
q_{i,\alpha} = W_{q,\alpha}h_i + b_{q,\alpha}\\
k_{i,\alpha} = W_{k,\alpha}h_i + b_{k,\alpha}
\end{align}
$\alpha$ means edit operation type, which includes \textit{Substitute} and \textit{Insert}, $q=(q_{1,\alpha},q_{2,\alpha},...,q_{n,\alpha})$ and $k=(k_{1,\alpha},k_{2,\alpha},...,k_{n,\alpha})$ are vector sequences.
$n$ means head size for multi-head attention.

As utterance order is important for dialogue, we use the RoPE \citep{su2021roformer} to provide relative position information in the utterances,
\begin{align}
s_{\alpha}(i,j)=(R_{i}q_{i,\alpha})^T(R_{j}k_{j,\alpha})
\end{align}
 where $R_i$ is a transformation matrix that satisfies the relation $R_i^TR_j=R_{j-i}$, and $s_{\alpha}(i,j)$ is our score.
 
During the decoding, any $s_{\alpha}(i,j)$ satisfies
\begin{align}
s_{\alpha}(i,j)=\left\{
\begin{array}{rcl}
1 & {s_{\alpha}(i,j) >= \theta}\\
0 & {s_{\alpha}(i,j) < \theta}
\label{con:decoding}
\end{array} \right.
\end{align}
where $\theta$ is a hyperparameter. 
% During our experiments, it is set to 0.1.


Since the distribution of edit operation matrix is severely unbalanced (most elements are equal to 0), we employed Circle Loss \citep{sun2020circle}, and tune it as Su\footnote{https://kexue.fm/archives/7359},

\begin{footnotesize}
\begin{align}
log(1+\sum_{(i,j)\in P_{\alpha}}e^{-s_{\alpha}(i,j)})+log(1+\sum_{(i,j)\in N_{\alpha}}e^{s_{\alpha}(i,j)})
\end{align}
\end{footnotesize}
\noindent
$P_{\alpha}$ is a set of the positive samples for edit operation type $\alpha$, $N_{\alpha}$ is a set of the negative samples.
% where $P_{\alpha}$ is a set of the positive character pair for edit operation type $\alpha$ in this instance, $N_{\alpha}$ is a set of the negative character pair for edit operation type $\alpha$ in this instance.
